Jointly Optimizing Query Encoder and Product Quantization to Improve Retrieval Performance

Recently, Information Retrieval community has witnessed fast-paced advances in Dense Retrieval (DR), which performs first-stage retrieval with embedding-based search. Despite the impressive ranking performance, previous studies usually adopt brute-force search to acquire candidates, which is prohibitive in practical Web search scenarios due to its tremendous memory usage and time cost. To overcome these problems, vector compression methods have been adopted in many practical embedding-based retrieval applications. One of the most popular methods is Product Quantization (PQ). However, although existing vector compression methods including PQ can help improve the efficiency of DR, they incur severely decayed retrieval performance due to the separation between encoding and compression. To tackle this problem, we present JPQ, which stands for Joint optimization of query encoding and Product Quantization. It trains the query encoder and PQ index jointly in an end-to-end manner based on three optimization strategies, namely ranking-oriented loss, PQ centroid optimization, and end-to-end negative sampling. We evaluate JPQ on two publicly available retrieval benchmarks. Experimental results show that JPQ significantly outperforms popular vector compression methods. Compared with previous DR models that use brute-force search, JPQ almost matches the best retrieval performance with 30x compression on index size. The compressed index further brings 10x speedup on CPU and 2x speedup on GPU in query latency.

==> notation.tex <==

\begin{table}[t]
    \centering
    \small
    \caption{The commonly used notions.}
    \label{tab:notions}
    \begin{tabular}{lll} \hlinew{0.8pt}
    \textbf{Notions} & \textbf{Type}& \textbf{Descriptions} 
    \\ \hline
    
    $q$             & text & A query. \\
    $d$             & text & A document.  \\
    $\mathcal{C}$   & set  & The set of all documents. \\
    $N$   			& $\mathbb{N}$  & The number of all documents. \\
    $\mathcal{D}^+_q$			& set & The positive documents for query $q$.\\
    $\mathcal{D}^-_q$			& set & The sampled negatives for query $q$.\\
    $f$           & func & The dual-encoders \\
    $\ell$   & func & The pair-wise loss \\
    $\vec{q}$   	& $\mathbb{R}^D$  & The query embedding output by $f$\\
    $\vec{d}$ 		& $\mathbb{R}^D$   & The document embedding output by $f$\\
   	$s(q,d)$        & $\mathbb{R}$ 	& The uncompressed relevance score\\
   	$n$        		& $\mathbb{N}$ 	& The number of returned documents \\
   	$M$             & $\mathbb{N}$ & The number of sub-vectors \\
   	$K$             & $\mathbb{N}$& The number of centroids per sub-vector \\
    $\vec{c}_{i,j}$ 		& $\mathbb{R}^{\frac{D}{m}}$& A PQ centroid embedding. \\
   	$\varphi_i(d) $  	& $\mathbb{N}$ & The $i_{th}$ PQ Index Assignment of $d$.\\
   	$\vec{d}^\dagger$		& $\mathbb{R}^D$ & The quantized document embedding. \\
	$\vec{q}_i$   	& $\mathbb{R}^\frac{D}{m}$  & The $i_{th}$ sub-vector of $\vec{q}$\\
   	$s^\dagger(q,d)$  & $\mathbb{R}$ & The relevance score computed by PQ \\
\hlinew{0.8pt} 
    \end{tabular}
\end{table}









==> results/cmp_exist_retrieve.tex <==
\begin{table*}
	\small
    \centering
    \robustify\bfseries% see 7.15 in siunitx.pdf
    \caption{
    Comparison with existing retrieval methods on TREC 2019 Deep Learning Track. */** denotes that JPQ performs significantly better than baselines at $p < 0.05/0.01$ level using the two-tailed pairwise t-test. }
    \label{tab:results_retriever}
    \begin{tabular}{@{}ll
    !{\color{lightgray}\vrule}
    S[table-format=3.2,table-column-width=11mm]
    S[table-format=1.3,table-column-width=12mm]S[table-format=1.3,table-column-width=12mm]S[table-format=1.3,table-column-width=12mm]S[table-format=1.3,table-column-width=12mm]
    !{\color{lightgray}\vrule}
    S[table-format=3.2,table-column-width=11mm]
    S[table-format=1.3,table-column-width=12mm]S[table-format=1.3,table-column-width=12mm]S[table-format=1.3,table-column-width=16mm]@{}}
    \toprule
    \textbf{} & \multirow{2}{*}{\textbf{Model}} 
    & {\textbf{Index}}
    & \multicolumn{2}{c}{\textbf{MARCO Passage}} & \multicolumn{2}{c!{\color{lightgray}\vrule}}{\textbf{DL Passage}} 
    & {\textbf{Index}}
    & \multicolumn{2}{c}{\textbf{MARCO Doc}} & {\textbf{DL Doc}} \\
     &  & GB & {MRR@10} & {R@100} & {NDCG@10} & {R@100} & GB & {MRR@100} & {R@100} & {NDCG@10} \\ \midrule
    \multicolumn{2}{l}{\textbf{Traditional BoW}} \\
     & BM25~\cite{yang2018anserini} & 0.59 & 0.187** & 0.670** & 0.497** & 0.460 & 2.17 & 0.278** & 0.807** & 0.523**  \\
    \multicolumn{2}{l}{\textbf{Augmented BoW}} \\
     & doc2query~\cite{nogueira2019document} & 0.65 & 0.215** & 0.713** & 0.533** & 0.471 & {n.a.} & {n.a.} & {n.a.} & {n.a.}  \\ 
     & DeepCT~\cite{dai2019context} & \bfseries 0.48 & 0.242** & 0.754** & 0.569** & 0.455 & {n.a.} & {n.a.} & {n.a.} & {n.a.}  \\ 
     & HDCT~\cite{Dai2020ContextAwareDT}  & {n.a.} & {n.a.} & {n.a.} & {n.a.} & {n.a.} &  1.71 & 0.319** & 0.843** & {n.a.} \\
     & docT5query~\cite{nogueira2019doc2query} & 0.96 & 0.272** & 0.819** & 0.642 & \bfseries 0.514 & 2.31 & 0.327** & 0.861** & 0.597  \\ 
    \multicolumn{2}{l}{\textbf{Brute-force DR}} \\
     & Rand Neg~\cite{huang2020embedding} & 25.34 & 0.301** & 0.853** & 0.612** & 0.464 & 9.20 & 0.330** & 0.859** & 0.572 \\
     & BM25 Neg~\cite{gao2020complementing} &  25.34 & 0.309** & 0.813** & 0.607** & 0.362** & 9.20 & 0.316** & 0.794** & 0.539*  \\
     & ANCE FirstP~\cite{xiong2020approximate} & 25.34 & 0.338 & 0.862 & 0.654 & 0.445* & 9.20 & 0.377** & 0.894** & 0.610 \\
     & ANCE MaxP~\cite{xiong2020approximate} & 25.34 & 0.338 & 0.862 & 0.654 & 0.445* & 58.91 & 0.380** & 0.903** & \bfseries 0.633 \\
     & TCT-ColBERT~\cite{lin2020distilling} & 25.34 & 0.335 & 0.859* & 0.670 & 0.459 & 58.91 & 0.332** & 0.866** & 0.612 \\
     & STAR~\cite{zhan2021optimizing} & 25.34 & 0.340 & 0.867 & 0.642 & 0.467 & 9.20 & 0.390** & 0.913 & 0.605  \\
     & ADORE+STAR~\cite{zhan2021optimizing} & 25.34 &  0.347 & \bfseries 0.876 &\bfseries 0.683 &  0.473 & 9.20 & 0.405  & 0.919 & 0.628 \\ 
    \multicolumn{2}{l}{\textbf{Late-Interaction}} \\
     & ColBERT~\cite{Khattab2020ColBERTEA} & 154 & \bfseries 0.360 & {n.a.} & {n.a.} & {n.a.} & 1500 & \bfseries 0.440 & \bfseries 0.923 & {n.a.} \\
    \multicolumn{2}{l}{\textbf{Ours}} \\
     & JPQ & 0.83 & 0.341 &  0.868 &  0.677 &  0.466 & \bfseries 0.30 &  0.401 &  0.914 &  0.623 \\ 
     % & JPQ Improv. Ratio & {\bfseries +8.72\%} & {\bfseries +5.00\%} & {\bfseries +10.26\%} & {\bfseries +8.19\%} & {\bfseries +9.15\%} & {\bfseries +4.31\%} & {\bfseries +5.88\%} \\ 
    \bottomrule
    \end{tabular}
    \end{table*}

==> results/new_cmp_exist_retrieve.tex <==
\begin{table*}
	\small
    \centering
    \robustify\bfseries% see 7.15 in siunitx.pdf
    \caption{
    Comparison with BoW models on TREC 2019 Deep Learning Track. */** denotes that JPQ performs significantly better than baselines at $p < 0.05/0.01$ level using the two-tailed pairwise t-test. }
    \label{tab:results_retriever}
    \begin{tabular}{@{}ll
    !{\color{lightgray}\vrule}
    S[table-format=1.2,table-column-width=11mm]
    S[table-format=1.3,table-column-width=12mm]S[table-format=1.3,table-column-width=12mm]S[table-format=1.3,table-column-width=12mm]S[table-format=1.3,table-column-width=12mm]
    !{\color{lightgray}\vrule}
    S[table-format=1.2,table-column-width=11mm]
    S[table-format=1.3,table-column-width=12mm]S[table-format=1.3,table-column-width=12mm]S[table-format=1.3,table-column-width=16mm]@{}}
    \toprule
    \textbf{} & \multirow{2}{*}{\textbf{Model}} 
    & {\textbf{Index}}
    & \multicolumn{2}{c}{\textbf{MARCO Passage}} & \multicolumn{2}{c!{\color{lightgray}\vrule}}{\textbf{DL Passage}} 
    & {\textbf{Index}}
    & \multicolumn{2}{c}{\textbf{MARCO Doc}} & {\textbf{DL Doc}} \\
     &  & GB & {MRR@10} & {R@100} & {NDCG@10} & {R@100} & GB & {MRR@100} & {R@100} & {NDCG@10} \\ \midrule
    \multicolumn{2}{l}{\textbf{Traditional BoW}} \\
     & BM25~\cite{yang2018anserini} & 0.59 & 0.187** & 0.670** & 0.497** & 0.460 & 2.17 & 0.278** & 0.807** & 0.523**  \\
    \multicolumn{2}{l}{\textbf{Augmented BoW}} \\
     & doc2query~\cite{nogueira2019document} & 0.65 & 0.215** & 0.713** & 0.533** & 0.471 & {n.a.} & {n.a.} & {n.a.} & {n.a.}  \\ 
     & DeepCT~\cite{dai2019context} & 0.48 & 0.242** & 0.754** & 0.569** & 0.455 & {n.a.} & {n.a.} & {n.a.} & {n.a.}  \\ 
     & HDCT~\cite{Dai2020ContextAwareDT}  & {n.a.} & {n.a.} & {n.a.} & {n.a.} & {n.a.} &  1.71 & 0.319** & 0.843** & {n.a.} \\
     & docT5query~\cite{nogueira2019doc2query} & 0.96 & 0.272** & 0.819** & 0.642 & \bfseries 0.514 & 2.31 & 0.327** & 0.861** & 0.597  \\ 
    \multicolumn{2}{l}{\textbf{Ours}} \\
     & JPQ & 0.83 & \bfseries 0.341 & \bfseries 0.868 & \bfseries 0.677 &  0.466 & 0.30 & \bfseries 0.401 & \bfseries 0.914 & \bfseries 0.623 \\ 
     % & JPQ Improv. Ratio & {\bfseries +8.72\%} & {\bfseries +5.00\%} & {\bfseries +10.26\%} & {\bfseries +8.19\%} & {\bfseries +9.15\%} & {\bfseries +4.31\%} & {\bfseries +5.88\%} \\ 
    \bottomrule
    \end{tabular}
    \end{table*}

\begin{table*}
	\small
    \centering
    \robustify\bfseries% see 7.15 in siunitx.pdf
    \caption{
    Comparison with previous DR models and late-interaction models on TREC 2019 Deep Learning Track. }
    \label{tab:results_retriever}
    \sisetup{input-decimal-markers = .,input-ignore = {,},group-separator={,}, group-four-digits = true, } % retain-explicit-plus
    \begin{tabular}{@{}ll
    !{\color{lightgray}\vrule}
    %S[table-format=3.0,table-column-width=11mm]
    S[table-format=2.0,table-column-width=11mm]<{x}
    S[table-format=2.0,table-column-width=12mm]<{\%}
    S[table-format=2.0,table-column-width=12mm]<{\%}
    S[table-format=2.0,table-column-width=12mm]<{\%}
    S[table-format=2.0,table-column-width=12mm]<{\%}
    !{\color{lightgray}\vrule}
    S[table-format=3.0,table-column-width=11mm]<{x}
    S[table-format=2.0,table-column-width=12mm]<{\%}
    S[table-format=2.0,table-column-width=12mm]<{\%}
    S[table-format=2.0,table-column-width=12mm]<{\%}L{0mm}
    @{}}
    \toprule
    \textbf{} & \multirow{2}{*}{\textbf{Model}} 
    & \multicolumn{1}{c}{\textbf{Index}}
    & \multicolumn{2}{c}{\textbf{MARCO Passage}} & \multicolumn{2}{c!{\color{lightgray}\vrule}}{\textbf{DL Passage}} 
    & \mc{\textbf{Index}}
    & \multicolumn{2}{c}{\textbf{MARCO Doc}} & \mc{\textbf{DL Doc}} \\
     &  & \mc{GB} & \mc{MRR@10} & \mc{R@100} & \mc{NDCG@10} & \mc{R@100} & \mc{GB} & \mc{MRR@100} & \mc{R@100} & \mc{NDCG@10} \\ \midrule
    & JPQ & \mc{0.83} & \mc{0.341} &  \mc{0.868} &  \mc{0.677} &  \mc{0.466} & \mc{0.30} &  \mc{0.401} &  \mc{0.914} &  \mc{0.623} \\ 
     \multicolumn{2}{l}{\textbf{Brute-force DR}} \\
     & Rand Neg~\cite{huang2020embedding} & +30 & -12 & -2 & -10 & -1 & +30 & -18 & -6 & -8 & \\
     & BM25 Neg~\cite{gao2020complementing} &  +30 & -9 & -6 & -10 & -22 & +30 & -21 & -13 & -13 & \\
     & ANCE FirstP~\cite{xiong2020approximate} & +30 & -1 & -1 & -4 & -5 & +30 & -6 & -2 & -2 & \\
     & ANCE MaxP~\cite{xiong2020approximate} & +30 & -1 & -1 & -4 & -5 & +196 & -5 & -1 & +2 & \\
     & TCT-ColBERT~\cite{lin2020distilling} & +30 & -2 & -1 & -1 & -2 & +196 & -17 & -5 & -2 & \\
     & STAR~\cite{zhan2021optimizing} & +30 & -0 & -0 & -5 & +0 & +30 & -3 & -0 & -3 & \\
     & ADORE+STAR~\cite{zhan2021optimizing} & +30 &  +2 & +1 & +1 & +2 & +30 & +1  & +1 & +1 & \\ 
    \multicolumn{2}{l}{\textbf{Late-Interaction}} \\
     & ColBERT~\cite{Khattab2020ColBERTEA} & \mc{186x} & +6 & \mc{n.a.} & \mc{n.a.} & \mc{n.a.} & \mc{5833x} & +10 &  +1 & \mc{n.a.} &\\
     % & JPQ Improv. Ratio & {\bfseries +8.72\%} & {\bfseries +5.00\%} & {\bfseries +10.26\%} & {\bfseries +8.19\%} & {\bfseries +9.15\%} & {\bfseries +4.31\%} & {\bfseries +5.88\%} \\ 
    \bottomrule
    \end{tabular}
    \end{table*}
    
    
\begin{table}
    \centering
    \small
    \caption{Comparison between late-interaction models and JPQ+BERT two-stage methods on MARCO Passage dataset.}
    \label{tab:comparison_with_e2e}
    \begin{tabular}{ll!{\color{lightgray}\vrule}ccc} \toprule
    & \textbf{Model} & \textbf{Latency (ms)} & \textbf{GPUs} & \textbf{MRR@10}
    \\ \midrule
    
	\multicolumn{2}{l}{\textbf{Late-Interaction}}  \\
	& {ColBERT}~\cite{Khattab2020ColBERTEA} & 458 & 4& 0.360  \\ 

	\multicolumn{2}{l}{\textbf{JPQ+$\text{BERT}_\text{base}$}}  \\
	& {Re-rank Top 10} & 116 & 1 & 0.367 \\
	& {Re-rank Top 30} & 187 & 1 & 0.378 \\
	\multicolumn{2}{l}{\textbf{JPQ+$\text{BERT}_\text{large}$}}  \\
	& {Re-rank Top 10} & 184 & 1 & 0.372 \\
	& {Re-rank Top 30} & 406 & 1 & \textbf{0.387} \\

	\bottomrule 
    \end{tabular}
\end{table}

%\begin{table}
%    \centering
%    \small
%    \caption{Comparison between late-interaction models and JPQ+BERT two-stage methods on MARCO Passage dataset. Latency is in milliseconds.}
%    \label{tab:comparison_with_e2e}
%    \begin{tabular}{ll!{\color{lightgray}\vrule}ccc!{\color{lightgray}\vrule}c} \toprule
%    & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c!{\color{lightgray}\vrule}}{\textbf{Passage}} & \textbf{Document} \\
%    & & \textbf{Latency} & \textbf{GPUs} & \textbf{MRR@10} & \textbf{MRR@100}\\ 
%    \midrule
%    
%	\multicolumn{2}{l}{\textbf{Late-Interaction}}  \\
%	& {ColBERT}~\cite{Khattab2020ColBERTEA} & 458 & 4& 0.360 & 0.440 \\ 
%
%	\multicolumn{2}{l}{\textbf{JPQ+$\text{BERT}_\text{base}$}}  \\
%	& {Re-rank Top 10} & 116 & 1 & 0.367 & 0.443 \\
%	& {Re-rank Top 30} & 187 & 1 & 0.378 & \textbf{0.461}\\
%	\multicolumn{2}{l}{\textbf{JPQ+$\text{BERT}_\text{large}$}}  \\
%	& {Re-rank Top 10} & 184 & 1 & 0.372 & {n.a.} \\
%	& {Re-rank Top 30} & 406 & 1 & \textbf{0.387} & {n.a.} \\
%
%	\bottomrule 
%    \end{tabular}
%\end{table}

    

==> results/tradeoff_linechart.tex <==







